LoopedWAM: Looped World Action Models for Elastic Inference

World action models (WAMs) couple generative video modeling with robotic action prediction but typically require large video and action transformers, limiting deployment efficiency. We present LoopedWAM, a compact WAM that recurrently applies a shared six-block core in each expert, executing 30 transformer layers while storing only 12 blocks per expert. To account for their asymmetric inference costs, the video and action experts can operate at different depths: visual features are computed once per query, whereas action computation repeats at every sampling step. We further propose elastic self-distillation, which trains a single elastic checkpoint, LoopedWAM-E, across action-depth and sampling-step budgets. With only 0.58B policy parameters and no robot pretraining, LoopedWAM achieves 96.1% success on LIBERO, 91.9% on RoboTwin 2.0, and 52.2% on RoboCasaGR1, while using $7.4\times$ less peak GPU memory than Fast-WAM under matched inference measurements. On LIBERO, LoopedWAM-E achieves 96.0% success in 27.6 ms or 95.2% in 24.7 ms on an H100, providing multiple accuracy-latency operating points from a single checkpoint; with two sampling steps and four action loops, it stays within 0.5 points of LoopedWAM on all three benchmarks. Ablations demonstrate that weight-shared depth preserves competitive performance, while aggressive action-depth reduction requires explicit budget-aware training. On a real AgileX PiPER arm, LoopedWAM succeeds in 71.3% of 80 trials across four tasks.

==> tables/a_elastic9_rows.tex <==
1 & 2 & 24 & 24.7 & 2.58 & 96.87 & 99.07 & 96.60 & 88.20 & 95.18 & +0.85 \\
\rowcolor{oursrow}2 & 2 & 36 & 27.6 & 2.68 & 97.80 & 99.13 & 97.80 & 89.20 & 95.98 & +1.45 \\
\rowcolor{oursrow}4 & 2 & 60 & 33.2 & 2.78 & 97.20 & 99.27 & 97.53 & 88.53 & 95.63 & +0.67 \\
1 & 5 & 60 & 33.3 & 2.62 & 97.40 & 98.80 & 95.80 & 88.93 & 95.23 & +0.70 \\
2 & 5 & 90 & 39.1 & 2.72 & 97.67 & 98.93 & 96.87 & 88.73 & 95.55 & +0.70 \\
1 & 10 & 120 & 47.9 & 2.65 & 97.27 & 99.27 & 96.07 & 88.73 & 95.33 & +1.65 \\
4 & 5 & 150 & 54.5 & 2.82 & 97.67 & 99.33 & 97.07 & 90.33 & 96.10 & +0.65 \\
2 & 10 & 180 & 59.9 & 2.75 & 97.53 & 99.00 & 96.60 & 89.53 & 95.67 & +1.83 \\
4 & 10 & 300 & 86.2 & 2.85 & 97.60 & 98.87 & 97.73 & 90.67 & 96.22 & +1.35 \\
\midrule
\multicolumn{3}{@{}l}{\method (teacher)} & 91.8 & 2.05 & 96.87 & 99.53 & 97.87 & 90.13 & 96.10 & -- \\


==> tables/a_elastic_rt_gr1_rows.tex <==
1 & 2 & 24 & 89.5 & 89.0 & 89.3 & 43.2 \\
\rowcolor{oursrow}2 & 2 & 36 & 90.6 & 90.6 & 90.6 & 51.6 \\
\rowcolor{oursrow}4 & 2 & 60 & 91.3 & 91.6 & 91.5 & 52.4 \\
1 & 5 & 60 & 89.3 & 89.6 & 89.4 & 47.4 \\
2 & 5 & 90 & 90.6 & 90.9 & 90.7 & 50.8 \\
1 & 10 & 120 & 89.2 & 89.7 & 89.5 & 46.8 \\
4 & 5 & 150 & 91.1 & 91.5 & 91.3 & 53.5 \\
2 & 10 & 180 & 90.4 & 90.9 & 90.7 & 50.8 \\
4 & 10 & 300 & 91.1 & 91.3 & 91.2 & 51.7 \\
\midrule
\multicolumn{3}{@{}l}{\method (teacher, (4, 10))} & 92.1 & 91.7 & 91.9 & 52.2 \\


==> tables/a_elastic_short_rows.tex <==
1 & 2 & 24.7 & 96.47 & 98.93 & 95.27 & 86.67 & 94.33 \\
2 & 2 & 27.6 & 96.40 & 99.27 & 95.67 & 86.80 & 94.53 \\
4 & 2 & 33.2 & 97.00 & 98.80 & 96.33 & 87.73 & 94.97 \\
1 & 5 & 33.3 & 97.07 & 99.07 & 96.53 & 85.47 & 94.53 \\
2 & 5 & 39.1 & 96.47 & 99.00 & 96.13 & 87.80 & 94.85 \\
1 & 10 & 47.9 & 96.73 & 98.60 & 93.87 & 85.53 & 93.68 \\
4 & 5 & 54.5 & 96.80 & 99.27 & 96.33 & 89.40 & 95.45 \\
2 & 10 & 59.9 & 96.40 & 98.47 & 95.20 & 85.27 & 93.83 \\
4 & 10 & 86.2 & 96.53 & 98.93 & 95.27 & 88.73 & 94.87 \\
\midrule
\multicolumn{2}{@{}l}{Specialist (1, 2)} & 23.4 & 96.20 & 98.53 & 95.33 & 85.00 & 93.77 \\
\multicolumn{2}{@{}l}{Teacher (4, 10)} & 99.3 & 96.93 & 98.73 & 96.13 & 87.87 & 94.92 \\


==> tables/a_elastic_untrained_rows.tex <==
1 & 96.73 & 98.60 & 93.87 & 85.53 & 93.68 \\
2 & 96.40 & 98.47 & 95.20 & 85.27 & 93.83 \\
3 & 96.80 & 99.07 & 95.53 & 85.20 & 94.15 \\
4 & 96.53 & 98.93 & 95.27 & 88.73 & 94.87 \\
5 & 96.27 & 98.93 & 96.80 & 88.13 & 95.03 \\
6 & 96.53 & 99.07 & 96.60 & 86.93 & 94.78 \\


==> tables/a_gr1_groups_rows.tex <==
GR00T-N1.6~\cite{bjorck2025gr00t} & -- & 24.2 & 56.9 & 51.9 & 55.1 & 57.6 & 47.6 \\
StarVLA~\cite{community2026starvla} & 50 & 50.3 & 52.8 & 38.0 & 39.2 & 58.5 & 47.8 \\
DiT4DiT~\cite{ma2026dit4dit} & 50 & 50.3 & 57.6 & 39.0 & 46.4 & 60.0 & 50.8 \\
ABot-M0~\cite{yang2026abot} & 50 & 61.7 & 61.6 & 51.0 & 56.8 & 58.0 & 58.3 \\
\midrule
\rowcolor{oursrow}\method & 50 & 52.7 & 55.2 & 46.5 & 48.8 & 57.5 & 52.2 \\
\rowcolor{oursrow}\methodE\ (4, 2) & 50 & 53.0 & 61.2 & 46.0 & 46.0 & 55.0 & 52.4 \\
\rowcolor{oursrow}\methodE\ (2, 2) & 50 & 51.0 & 53.2 & 47.0 & 50.4 & 56.5 & 51.6 \\


==> tables/a_gr1_tasks_rows.tex <==
Bottle $\to$ cabinet, close & 58.0 & 62.0 & 58.0 \\
Can $\to$ drawer, close & 68.0 & 76.0 & 70.0 \\
Cup $\to$ drawer, close & 44.0 & 34.0 & 48.0 \\
Milk $\to$ microwave, close & 48.0 & 50.0 & 46.0 \\
Potato $\to$ microwave, close & 44.0 & 42.0 & 36.0 \\
Wine $\to$ cabinet, close & 54.0 & 54.0 & 48.0 \\
\textit{PnP + close (6)} & \textit{52.7} & \textit{53.0} & \textit{51.0} \\
\midrule
Cutting board $\to$ basket & 66.0 & 58.0 & 52.0 \\
Cutting board $\to$ cardboard box & 38.0 & 58.0 & 44.0 \\
Cutting board $\to$ pan & 68.0 & 66.0 & 80.0 \\
Cutting board $\to$ pot & 56.0 & 62.0 & 54.0 \\
Cutting board $\to$ tiered basket & 48.0 & 62.0 & 36.0 \\
\textit{Cutting board (5)} & \textit{55.2} & \textit{61.2} & \textit{53.2} \\
\midrule
Placemat $\to$ basket & 40.0 & 48.0 & 56.0 \\
Placemat $\to$ bowl & 58.0 & 68.0 & 52.0 \\
Placemat $\to$ plate & 64.0 & 42.0 & 50.0 \\
Placemat $\to$ tiered shelf & 24.0 & 26.0 & 30.0 \\
\textit{Placemat (4)} & \textit{46.5} & \textit{46.0} & \textit{47.0} \\
\midrule
Tray $\to$ cardboard box & 54.0 & 40.0 & 56.0 \\
Tray $\to$ plate & 54.0 & 62.0 & 58.0 \\
Tray $\to$ pot & 56.0 & 54.0 & 56.0 \\
Tray $\to$ tiered basket & 52.0 & 44.0 & 50.0 \\
Tray $\to$ tiered shelf & 28.0 & 30.0 & 32.0 \\
\textit{Tray (5)} & \textit{48.8} & \textit{46.0} & \textit{50.4} \\
\midrule
Plate $\to$ bowl & 58.0 & 66.0 & 60.0 \\
Plate $\to$ cardboard box & 44.0 & 42.0 & 44.0 \\
Plate $\to$ pan & 48.0 & 52.0 & 42.0 \\
Plate $\to$ plate & 80.0 & 60.0 & 80.0 \\
\textit{Plate (4)} & \textit{57.5} & \textit{55.0} & \textit{56.5} \\
\midrule
Average (24 tasks) & 52.17 & 52.42 & 51.58 \\


==> tables/a_init_rows.tex <==
Blocks 10--15 (default) & 96.93 & 98.73 & 96.13 & 87.87 & 94.92 \\
Blocks 16--21 & 96.20 & 97.27 & 94.60 & 84.40 & 93.12 \\
Every 4th block (5, 9, \ldots, 25) & 94.93 & 95.73 & 93.87 & 81.33 & 91.47 \\
Mean of 4 blocks per slot & 96.27 & 96.47 & 94.40 & 84.13 & 92.82 \\
FFN units by weight magnitude & 95.80 & 98.27 & 92.93 & 81.47 & 92.12 \\
Random core & 92.00 & 91.07 & 85.13 & 60.60 & 82.20 \\
No video pretraining & 91.93 & 92.60 & 90.00 & 68.07 & 85.65 \\


==> tables/a_loops_rows.tex <==
Dense-12 & -- & -- & 0.58B & 40.8 & 94.80 & 93.27 & 92.13 & 79.73 & 89.98 & 77.25 \\
\method & 1 & 4 & 0.58B & 86.4 & 96.00 & 97.80 & 94.73 & 78.20 & 91.68 & 79.55 \\
\method & 2 & 2 & 0.58B & 58.3 & 96.93 & 96.53 & 94.27 & 82.07 & 92.45 & 78.90 \\
\method & 4 & 1 & 0.58B & 48.3 & 96.27 & 98.07 & 95.40 & 86.27 & 94.00 & 80.95 \\
\method, KV-mix & 4 & 1 & 0.58B & 50.9 & 97.40 & 98.33 & 96.93 & 85.13 & 94.45 & -- \\
\method & 4 & 2 & 0.58B & 67.2 & 96.93 & 98.80 & 95.33 & 87.07 & 94.53 & 82.40 \\
\method & 4 & 4 & 0.58B & 99.3 & 96.93 & 98.73 & 96.13 & 87.87 & 94.92 & 81.40 \\
Dense-30 & -- & -- & 1.42B & 90.5 & 97.27 & 98.60 & 95.87 & 90.80 & 95.63 & 83.60 \\


==> tables/a_loss_rows.tex <==
\methodE{} (\cref{eq:elastic}) & 95.98 & 95.63 & 95.33 & 95.65 & -- & 80.30 & 81.25 & 75.30 & 78.95 & -- \\
\midrule
Teacher trajectory & 95.26 & 95.98 & 95.08 & 95.44 & $-0.21$ & 78.95 & 80.55 & 73.75 & 77.75 & $-1.20$ \\
w/o $\mathcal{L}_{\text{anchor}}$ & 95.58 & 95.50 & 94.88 & 95.32 & $-0.33$ & 78.70 & 80.75 & 75.40 & 78.28 & $-0.67$ \\
w/o $\mathcal{L}_{\text{end}}$ & 95.93 & 95.65 & 94.78 & 95.45 & $-0.20$ & 78.50 & 81.10 & 76.05 & 78.55 & $-0.40$ \\
w/o $\mathcal{L}_{\text{grip}}$ & 95.88 & 95.38 & 95.25 & 95.50 & $-0.15$ & \multicolumn{5}{c}{n/a (continuous grippers)} \\
\midrule
Teacher, $(4,10)$ & \multicolumn{3}{c}{96.10} & -- & -- & \multicolumn{3}{c}{81.40} & -- & -- \\

==> tables/a_naive_rows.tex <==
1 & 18.73 & 25.13 & 5.07 & 0.27 & 12.30 \\
2 & 65.07 & 72.13 & 54.60 & 30.47 & 55.57 \\
3 & 95.53 & 92.60 & 92.93 & 76.80 & 89.47 \\
4 & 96.93 & 98.73 & 96.13 & 87.87 & 94.92 \\
5 & 94.47 & 98.87 & 96.20 & 88.87 & 94.60 \\
6 & 88.13 & 96.93 & 93.73 & 78.00 & 89.20 \\


==> tables/a_part_rows.tex <==
3/6/3 & 4 & 1--3 / 10--15 / 28--30 & 96.93 & 98.73 & 96.13 & 87.87 & 94.92 \\
0/6/6 & 4 & -- / 13--18 / 25--30 & 97.20 & 98.73 & 95.27 & 86.47 & 94.42 \\
1/6/5 & 4 & 1 / 13--18 / 26--30 & 97.27 & 98.13 & 95.93 & 83.33 & 93.67 \\
5/6/1 & 4 & 1--5 / 13--18 / 30 & 96.73 & 97.40 & 93.60 & 84.93 & 93.17 \\
6/6/0 & 4 & 1--6 / 13--18 / -- & 95.07 & 92.67 & 91.27 & 82.07 & 90.27 \\
1/9/2 & 3 & 1 / 11--19 / 29--30 & 97.53 & 98.33 & 93.47 & 77.80 & 91.78 \\
4/3/5 & 7 & 1--4 / 14--16 / 26--30 & 93.33 & 97.87 & 92.47 & 79.33 & 90.75 \\


==> tables/a_rt10_tasks_rows.tex <==
\texttt{adjust\_bottle} & 99.5 & 99.5 & 99.5 & 99.0 & 100.0 & 99.5 & 99.5 \\
\texttt{grab\_roller} & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 99.5 \\
\texttt{stack\_blocks\_two} & 98.0 & 97.5 & 98.0 & 99.0 & 97.0 & 97.5 & 100.0 \\
\texttt{press\_stapler} & 90.5 & 88.5 & 91.0 & 84.5 & 85.0 & 92.5 & 91.5 \\
\texttt{stamp\_seal} & 87.0 & 83.0 & 90.0 & 89.0 & 91.5 & 89.5 & 93.5 \\
\texttt{scan\_object} & 79.5 & 83.0 & 87.0 & 83.0 & 85.5 & 84.5 & 91.0 \\
\texttt{move\_stapler\_pad} & 61.0 & 63.5 & 63.5 & 75.5 & 69.5 & 72.5 & 80.0 \\
\texttt{turn\_switch} & 59.5 & 61.5 & 62.0 & 64.0 & 67.0 & 74.5 & 66.0 \\
\texttt{hanging\_mug} & 44.5 & 45.5 & 40.0 & 45.0 & 51.0 & 58.5 & 59.5 \\
\texttt{open\_microwave} & 53.0 & 73.5 & 58.0 & 70.5 & 77.5 & 45.0 & 55.5 \\
\midrule
Average & 77.25 & 79.55 & 78.90 & 80.95 & 82.40 & 81.40 & 83.60 \\


==> tables/a_rt50_tasks_rows.tex <==
\texttt{adjust\_bottle} & 100 & 99 & 99.5 & \texttt{place\_can\_basket} & 61 & 57 & 59.0 \\
\texttt{beat\_block\_hammer} & 100 & 96 & 98.0 & \texttt{place\_cans\_plasticbox} & 99 & 96 & 97.5 \\
\texttt{blocks\_ranking\_rgb} & 99 & 99 & 99.0 & \texttt{place\_container\_plate} & 96 & 97 & 96.5 \\
\texttt{blocks\_ranking\_size} & 98 & 96 & 97.0 & \texttt{place\_dual\_shoes} & 91 & 89 & 90.0 \\
\texttt{click\_alarmclock} & 99 & 100 & 99.5 & \texttt{place\_empty\_cup} & 100 & 100 & 100.0 \\
\texttt{click\_bell} & 100 & 100 & 100.0 & \texttt{place\_fan} & 96 & 93 & 94.5 \\
\texttt{dump\_bin\_bigbin} & 100 & 98 & 99.0 & \texttt{place\_mouse\_pad} & 96 & 95 & 95.5 \\
\texttt{grab\_roller} & 100 & 100 & 100.0 & \texttt{place\_object\_basket} & 86 & 82 & 84.0 \\
\texttt{handover\_block} & 94 & 95 & 94.5 & \texttt{place\_object\_scale} & 98 & 97 & 97.5 \\
\texttt{handover\_mic} & 100 & 100 & 100.0 & \texttt{place\_object\_stand} & 92 & 97 & 94.5 \\
\texttt{hanging\_mug} & 57 & 45 & 51.0 & \texttt{place\_phone\_stand} & 99 & 99 & 99.0 \\
\texttt{lift\_pot} & 100 & 100 & 100.0 & \texttt{place\_shoe} & 96 & 98 & 97.0 \\
\texttt{move\_can\_pot} & 93 & 99 & 96.0 & \texttt{press\_stapler} & 97 & 98 & 97.5 \\
\texttt{move\_pillbottle\_pad} & 100 & 100 & 100.0 & \texttt{put\_bottles\_dustbin} & 90 & 89 & 89.5 \\
\texttt{move\_playingcard\_away} & 100 & 100 & 100.0 & \texttt{put\_object\_cabinet} & 91 & 87 & 89.0 \\
\texttt{move\_stapler\_pad} & 93 & 85 & 89.0 & \texttt{rotate\_qrcode} & 82 & 80 & 81.0 \\
\texttt{open\_laptop} & 92 & 93 & 92.5 & \texttt{scan\_object} & 85 & 88 & 86.5 \\
\texttt{open\_microwave} & 36 & 50 & 43.0 & \texttt{shake\_bottle} & 100 & 100 & 100.0 \\
\texttt{pick\_diverse\_bottles} & 86 & 85 & 85.5 & \texttt{shake\_bottle\_horizontally} & 100 & 100 & 100.0 \\
\texttt{pick\_dual\_bottles} & 100 & 96 & 98.0 & \texttt{stack\_blocks\_three} & 97 & 96 & 96.5 \\
\texttt{place\_a2b\_left} & 97 & 94 & 95.5 & \texttt{stack\_blocks\_two} & 100 & 100 & 100.0 \\
\texttt{place\_a2b\_right} & 96 & 92 & 94.0 & \texttt{stack\_bowls\_three} & 79 & 83 & 81.0 \\
\texttt{place\_bread\_basket} & 93 & 94 & 93.5 & \texttt{stack\_bowls\_two} & 95 & 96 & 95.5 \\
\texttt{place\_bread\_skillet} & 89 & 87 & 88.0 & \texttt{stamp\_seal} & 98 & 96 & 97.0 \\
\texttt{place\_burger\_fries} & 97 & 98 & 97.5 & \texttt{turn\_switch} & 60 & 70 & 65.0 \\


==> tables/t_abl_init_rows.tex <==
\rowcolor{oursrow}Blocks 10--15 (default) & 94.9 & -- \\
Blocks 16--21 & 93.1 & $-$1.8 \\
Every 4th block & 91.5 & $-$3.4 \\
Random core & 82.2 & $-$12.7 \\
No video pretraining & 85.7 & $-$9.2 \\


==> tables/t_abl_loops_rows.tex <==
Dense-12 & -- & -- & 0.58B & 90.0 & 77.3 \\
\method & 1 & 4 & 0.58B & 91.7 & 79.6 \\
\method & 2 & 2 & 0.58B & 92.5 & 78.9 \\
\method & 4 & 1 & 0.58B & 94.0 & 81.0 \\
\method & 4 & 2 & 0.58B & 94.5 & 82.4 \\
\rowcolor{oursrow}\method & 4 & 4 & 0.58B & 94.9 & 81.4 \\
Dense-30 & -- & -- & 1.42B & 95.6 & 83.6 \\


==> tables/t_abl_part_rows.tex <==
\rowcolor{oursrow}3/6/3 & 4 & 94.9 & -- \\
0/6/6 & 4 & 94.4 & $-$0.5 \\
6/6/0 & 4 & 90.3 & $-$4.6 \\
1/9/2 & 3 & 91.8 & $-$3.1 \\
4/3/5 & 7 & 90.8 & $-$4.1 \\


==> tables/t_eff_rows.tex <==
\multicolumn{9}{@{}l}{\textit{Prior world action models}} \\
Fast-WAM$^{*}$ & $\sim$6B & -- & 10 & 15.25 & 107.5 & 1.0$\times$ & 96.6 & 91.8 \\
Fast-WAM$^{*}$ & $\sim$6B & -- & 2 & 15.32 & 37.1 & 2.9$\times$ & 96.0 & 90.1 \\
Faster-WAM$^{*}$ & $\sim$6.3B & -- & 10 & 12.76 & 72.6 & 1.5$\times$ & 98.7 & 92.6 \\
Light-WAM$^{*}$ & 1.9B & -- & -- & 4.38 & 21.8 & 4.9$\times$ & 95.8 & 76.4 \\
\midrule
\multicolumn{9}{@{}l}{\textit{Dense controls (same Wan2.1 donor)}} \\
Dense-30 & 1.42B & -- & 10 & 3.79 & 90.5 & 1.2$\times$ & 96.3 & -- \\
Dense-30-E & 1.42B & -- & 2 & 4.33 & 33.9 & 3.2$\times$ & 95.9 & -- \\
Dense-12 & 0.58B & -- & 10 & 2.09 & 40.8 & 2.6$\times$ & 94.0 & -- \\
\midrule
\rowcolor{oursrow}\method & 0.58B & 4 & 10 & 2.05 & 91.8 & 1.2$\times$ & 96.1 & 91.9 \\
\rowcolor{oursrow}\method & 0.58B & 4 & 2 & 2.09 & 35.0 & 3.1$\times$ & 95.3 & 91.2 \\
\rowcolor{oursrow}\methodE & 0.58B & 4 & 2 & 2.78 & 33.2 & 3.2$\times$ & 95.6 & 91.5 \\
\rowcolor{oursrow}\methodE & 0.58B & 2 & 2 & 2.68 & 27.6 & 3.9$\times$ & 96.0 & 90.6 \\
\rowcolor{oursrow}\methodE & 0.58B & 1 & 2 & 2.58 & 24.7 & 4.4$\times$ & 95.2 & 89.3 \\


==> tables/t_gr1_rows.tex <==
GR00T-N1.6$^{\ddagger}$~\cite{bjorck2025gr00t} & 3.3B & 47.6 \\
StarVLA-GR00T~\cite{community2026starvla} & 4B & 47.8 \\
DiT4DiT~\cite{ma2026dit4dit} & -- & 50.8 \\
Being-H0.7~\cite{luo2026being} & 3B & 49.2 \\
LDA-1B$^{\S}$~\cite{lyu2026lda} & 1.6B & 55.4 \\
THAW-VLA$^{\dagger}$~\cite{dao2026thawvla} & 0.8B & 50.5 \\
VP-VLA~\cite{wang2026vp} & $2\times4$B & 53.8 \\
TwinBrainVLA~\cite{yu2026twinbrainvla} & $2\times4$B & 54.6 \\
ABot-M0~\cite{yang2026abot} & 4B & 58.3 \\
ACE-Ego-0~\cite{li2026ace} & 4B & 72.8 \\
\midrule
\rowcolor{oursrow}\textbf{\method} & 0.58B & 52.2 \\
\rowcolor{oursrow}\methodE\ ($K_a{=}4$, $N{=}2$) & 0.58B & 52.4 \\
\rowcolor{oursrow}\methodE\ ($K_a{=}2$, $N{=}2$) & 0.58B & 51.6 \\


==> tables/t_libero_rows.tex <==
OpenVLA-OFT~\cite{kim2025fine} & 7B & \cmark & 97.6 & 98.4 & 97.9 & 94.5 & 97.1 \\
$\pi_0$~\cite{black2024pi_0} & 3.3B & \cmark & 96.8 & 98.8 & 95.8 & 85.2 & 94.2 \\
$\pi_{0.5}$~\cite{intelligence2025pi_} & 3B & \cmark & 98.8 & 98.2 & 98.0 & 92.4 & 96.9 \\
GR00T-N1.6~\cite{bjorck2025gr00t} & 3.3B & \cmark & 97.7 & 98.5 & 97.5 & 94.4 & 97.0 \\
SmolVLA~\cite{shukor2025smolvla} & 0.45B & \xmark & 90.0 & 96.0 & 92.0 & 71.0 & 87.3 \\
RD-VLA~\cite{tur2026recurrent} & 0.5B & -- & 92.0 & 99.0 & 96.0 & 84.8 & 93.0 \\
\midrule
Motus~\cite{bi2026motus} & 8B & \cmark & 96.8 & 99.8 & 96.6 & 97.6 & 97.7 \\
LingBot-VA~\cite{li2026causal} & 5.3B & \cmark & 98.5 & 99.6 & 97.2 & 98.5 & 98.5 \\
Cosmos Policy~\cite{kim2026cosmos} & 2B & \xmark & 98.1 & 100.0 & 98.2 & 97.6 & 98.5 \\
LaWAM~\cite{chen2026lawam} & 2.3B & \cmark & 99.4 & 99.6 & 98.4 & 97.0 & 98.6 \\
LiLa-WAM~\cite{yang2026lila} & 0.5B & \xmark & 98.0 & 98.8 & 97.2 & 94.2 & 97.1 \\
Light-WAM$^{*}$~\cite{li2026light} & 1.9B & \xmark & 96.7 & 98.9 & 96.6 & 90.9 & 95.8 \\
Fast-WAM$^{*}$~\cite{yuan2026fast} & $\sim$6B & \xmark & 97.5 & 99.3 & 96.3 & 93.5 & 96.6 \\
Faster-WAM$^{*}$~\cite{zhao2026faster} & $\sim$6.3B & \xmark & 99.0 & 99.6 & 98.2 & 98.1 & 98.7 \\
\midrule
\rowcolor{oursrow}\textbf{\method} & 0.58B & \xmark & 96.9 & 99.5 & 97.9 & 90.1 & 96.1 \\
\rowcolor{oursrow}\methodE\ ($K_a{=}4$, $N{=}2$) & 0.58B & \xmark & 97.2 & 99.3 & 97.5 & 88.5 & 95.6 \\
\rowcolor{oursrow}\methodE\ ($K_a{=}2$, $N{=}2$) & 0.58B & \xmark & 97.8 & 99.1 & 97.8 & 89.2 & 96.0 \\


==> tables/t_robotwin_rows.tex <==
$\pi_0$~\cite{black2024pi_0} & 3.3B & \cmark & 65.9 & 58.4 & 62.2 \\
$\pi_{0.5}$~\cite{intelligence2025pi_} & 3B & \cmark & 82.7 & 76.8 & 79.8 \\
X-VLA~\cite{zheng2026x} & 0.9B & \cmark & 72.8 & 72.8 & 72.8 \\
\midrule
Motus~\cite{bi2026motus} & 8B & \cmark & 88.7 & 87.0 & 87.8 \\
LingBot-VA~\cite{li2026causal} & 5.3B & \cmark & 92.9 & 91.6 & 92.2 \\
AHA-WAM~\cite{cai2026aha} & 7.2B & \xmark & 93.4 & 92.2 & 92.8 \\
Fast-WAM~\cite{yuan2026fast} & $\sim$6B & \xmark & 91.9 & 91.8 & 91.8 \\
Faster-WAM~\cite{zhao2026faster} & $\sim$6.3B & \xmark & 92.8 & 92.3 & 92.6 \\
LaWAM~\cite{chen2026lawam} & 2.3B & \cmark & 92.6 & 89.8 & 91.2 \\
Efficient-WAM~\cite{li2026efficient} & 1B & \xmark & 86.7 & 85.7 & 86.2 \\
Light-WAM~\cite{li2026light} & 1.9B & \xmark & 76.4 & 76.3 & 76.4 \\
LiLa-WAM~\cite{yang2026lila} & 0.5B & \xmark & 90.5 & 89.0 & 89.8 \\
\midrule
\rowcolor{oursrow}\textbf{\method} & 0.58B & \xmark & 92.1 & 91.7 & 91.9 \\
\rowcolor{oursrow}\methodE\ ($K_a{=}4$, $N{=}2$) & 0.58B & \xmark & 91.3 & 91.6 & 91.5 \\
\rowcolor{oursrow}\methodE\ ($K_a{=}2$, $N{=}2$) & 0.58B & \xmark & 90.6 & 90.6 & 90.6 \\

